rVAD: An Unsupervised Segment-Based Robust Voice Activity Detection Method

This paper presents an unsupervised segment-based method for robust voice activity detection (rVAD). The method consists of two passes of denoising followed by a voice activity detection (VAD) stage. In the first pass, high-energy segments in a speech signal are detected by using a posteriori signal-to-noise ratio (SNR) weighted energy difference and if no pitch is detected within a segment, the segment is considered as a high-energy noise segment and set to zero. In the second pass, the speech signal is denoised by a speech enhancement method, for which several methods are explored. Next, neighbouring frames with pitch are grouped together to form pitch segments, and based on speech statistics, the pitch segments are further extended from both ends in order to include both voiced and unvoiced sounds and likely non-speech parts as well. In the end, a posteriori SNR weighted energy difference is applied to the extended pitch segments of the denoised speech signal for detecting voice activity. We evaluate the VAD performance of the proposed method using two databases, RATS and Aurora-2, which contain a large variety of noise conditions. The rVAD method is further evaluated, in terms of speaker verification performance, on the RedDots 2016 challenge database and its noise-corrupted versions. Experiment results show that rVAD is compared favourably with a number of existing methods. In addition, we present a modified version of rVAD where computationally intensive pitch extraction is replaced by computationally efficient spectral flatness calculation. The modified version significantly reduces the computational complexity at the cost of moderately inferior VAD performance, which is an advantage when processing a large amount of data and running on low resource devices. The source code of rVAD is made publicly available.

==> Reference <==
@Article{Martin2001a,
author={R. Martin},
title={{N}oise power spectral density estimation based on optimal smoothing and minimum statistics},
journal={IEEE Transactions on Speech and Audio Processing},
volume={9},
number ={5},
pages={504-512},
year={2001}
}

@INPROCEEDINGS{kraljevski2015comparison,
  title={Comparison of forced-alignment speech recognition and humans for generating reference VAD},
  author={Kraljevski, Ivan and Tan, Zheng-Hua and Bissiri, Maria Paola},
  booktitle ={Proc. of Interspeech},
  year={2015},
  pages= {2937-941}
  }

@Article{Cohen2002a,
author={I. Cohen and B. Berdugo},
title={{N}oise Estimation by Minima Controlled Recursive Averaging for Robust Speech Enhancement},
journal= {IEEE Signal Processing Letters},
volume ={9},
number ={1},
pages={12-15},
year={2002}
}

@Article{Boll1979a,
author={S. Boll},
title={{S}uppression of acoustic noise in speech using spectral subtraction},
journal={IEEE Trans. on Acoustics, Speech, and Signal Processing},
volume={27},
number={2},
pages={113-120},
year={1979}
}

@Article{Xu2008a,
author={H. Xu and Z.-H. Tan and P. Dalsgaard and B. Lindberg},
title={{R}obust Speech Recognition by Non-Local Means De-Noising Processing},
journal={IEEE Signal Processing Letters},
volume={15},
pages={701- 704},
year={2008}
}


@INPROCEEDINGS{Renevey2001a,
    author = {Andrzej Drygajlo},
    title = {Entropy based voice activity detection in very noisy conditions},
    booktitle = {Proc. of EUROSPEECH},
    year = {2001},
    pages = {1887-1890}
}


@Article{Vlaj2005a,
author={D. Vlaj and B. Kotnik and B. Horvat and Z. Kacic},
title={{A} computationally efficient mel-filter bank VAD algorithm for distributed speech recognition systems},
journal={EURASIP Journal of Applied Signal Processing},
volume={2005},
number={4},
pages={487-497},
year={2005}
}

@Article{Madhu2009,
author={N. Madhu},
title={{N}ote on measures for spectral flatness},
 journal={Electronics Letters},
 volume={45},
number ={23},
  pages={1195 - 1196},
  year={2009}
 }

@INPROCEEDINGS{Dong2002a,
author={ D. Enqing and L. Guizhong and Z. Yatong and Z. Xiaodi},
title={{A}pplying support vector machines to voice activity detection},
booktitle={Proc. of International Conference on Spoken Language Processing},
year={2002}
}
 
@Article{Sohn1999a,
author={J. Sohn and N. S. Kim and W. Sung},
title={{A} statistical model-based voice activity detection},
journal={IEEE Signal Processing Letters},
volume={6},
number = {1},
pages={1-3},
year={1999}
}

@misc{ETSI2007,
author = {{ETSI}},
title={{S}peech processing, transmission and quality aspects ({STQ}): Distributed speech recognition, advanced front-end feature extraction algorithm, compression algorithm {ES} 202 050 v1.1.5, {ETSI}, {G}eneve, 2007}
}

@misc{ETSI2002,
author={{ETSI} },
title={{S}peech processing, transmission and quality aspects ({STQ}): Distributed speech recognition, advanced front-end feature extraction algorithm, compression algorithm {ES} 202 050 v1.1.1, {ETSI}, {G}eneve, 2002}
}


@Article{Ghosh2011,
author={P. Ghosh and A. Tsiartas and S. Narayanan},
title={{R}obust voice activity detection using long-term signal variability},
journal={IEEE Trans Audio Speech Lang Process},
volume={19},
number ={3},
pages={600-613},
year={2011}
}

@INPROCEEDINGS{Povey_ASRU2011,
         author = {Povey, Daniel and Ghoshal, Arnab and Boulianne, Gilles and Burget, Lukas and Glembek, Ondrej and Goel, Nagendra and Hannemann, Mirko and Motlicek, Petr and Qian, Yanmin and Schwarz, Petr and Silovsky, Jan and Stemmer, Georg and Vesely, Karel},
           title = {The Kaldi Speech Recognition Toolkit},
      booktitle = {Proc. of IEEE Workshop on Automatic Speech Recognition and Understanding},
           year = {2011},
     }


@Article{Vlaj2012,
author={D. Vlaj and Z. Kačič and M. Kos},
title={{V}oice activity detection algorithm using nonlinear spectral weights, hangover and hang before criteria},
journal={Computers \& Electrical Engineering},
volume ={38},
number ={6},
pages={1820-1836},
year={2012}
}

@INPROCEEDINGS{Walker2012,
author ={K. Walker and S. Strassel},
title={{T}he RATS radio traffic collection system},
booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
year={2012},
pages= {291-297}
}

@Article{zt2010,
author = {Z.-H. Tan and B. Lindberg},
title={{L}ow-Complexity Variable Frame Rate Analysis for Speech Recognition and Voice Activity Detection},
journal = {IEEE Journal of Selected Topics in Signal Processing},
volume ={4},
number ={5},
pages = {798 - 807},
year={2010}
}

@online{Boersma2009,
author ={P. Boersma and D. Weenink},
title ={{P}raat: doing phonetics by computer (Version 5.1.05) [Computer program]},
url = {http://www.praat.org/},
year ={2009},
note = "[Online; Accessed 2009]"
}

@online{NISTSAD2015,
author ={},
title = {{E}valuation Plan for the NIST Open Evaluation of Speech Activity Detection (OpenSAD15)},
url= {https://www.nist.gov/itl/iad/mig/nist-open-speech-activity-detection-evaluation},
year = {2015}
}



@book{Segura2006,
author ={A. M. Peinado and J. C. Segura},
title ={{S}tandards for Distributed Speech Recognition, in Speech Recognition Over Digital Channels: Robustness and Standards},
publisher = {John Wiley \& Sons, Ltd},
address ={Chichester, UK.}
}

@INPROCEEDINGS{Ng2012a,
author ={T. Ng and B. Zhang and L. Nguyen and S. Matsoukas and X. Zhou and  N. Mesgarani and K. Veselý and P. Matejka},
title = {{D}eveloping a Speech Activity Detection System for the DARPA RATS Program},
booktitle={Proc. of Interspeech},
pages={1969-1972},
year = {2012}
}

@techreport{ITU1996a,
author ={ITU},
title = {{C}oding of speech at 8 kbit/s using conjugate structure algebraic code-excited linear-prediction (CS-ACELP) Annex B: A silence compression scheme},
institution ={ ITU Recommendation G.729, Geneve},
year = {1996}
}

@techreport{ITU1996b,
author = {ITU},
title ={{D}ual rate speech coder for multimedia communications transmitting at 5.3 and 6.3 kbit/s. Annex A: Silence compression scheme},
institution ={ITU Recommendation G.723.1, Geneve},
year= {1996}
}

@INPROCEEDINGS{Fujimoto2008a,
author= {M. Fujimoto and K. Ishizuka and T. Nakatani},
title ={{A} voice activity detection based on the adaptive integration of multiple speech features and a signal decision scheme},
 booktitle ={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 year={2008}
 }
 
@Article{Petsatodis2011a,
author ={T. Petsatodis and C. Boukis and F. Talantzis and Z.-H. Tan and R. Prasad},
title = {{C}onvex Combination of Multiple Statistical Models with Application to VAD},
journal = {IEEE Transactions on Audio, Speech and Language Processing},
volume = {19},
number ={8},
pages = {2314-2327},
year = { 2011}
}

@INPROCEEDINGS{Shah2004a,
author = {J. Shah and A. Iyer and B. Smolenski and R. Yantorno},
title = {{R}obust voiced/unvoiced classification using novel features and Gaussian mixture model},
booktitle = {Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year = {2004}
}

@INPROCEEDINGS{Shin2002a,
author = {W.-H. Shin and  B.-S. Lee, and  Y.-K. Lee and J.-S. Lee},
title = {{S}peech/non-speech classification using multiple features for robust endpoint detection},
booktitle = {Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year= {2002}
} 

@Article{Shin2010b,
author = {J. W. Shin and  J.-H. Chang and N. S. Kim},
title ={{V}oice activity detection based on statistical models and machine learning approaches},
journal ={Computer Speech \& Language},
volume = {24},
number = {3},
pages = {515-530},
year = {2010}
}

@Article{Ramirez2004a,
author ={ J. Ramirez and C. Segura and C. Benitez and A. Torre and A. Rubio},
title ={{A} new Kullback-Leibler VAD for speech recognition in noise},
journal ={IEEE Signal Processing Letters},
volume ={11},
number ={2},
pages={266-269},
year = {2004}
}

@techreport{Peeters2004,
author = {G. Peeters},
title ={{A} large set of audio features for sound description (similarity and classification)},
institution ={CUIDADO project},
year = {2004}
}

@Article{Johnston1988,
author = {J. D. Johnston},
title={{T}ransform coding of audio signals using perceptual noise criteria},
journal={IEEE Journal on Selected Areas in Communications},
volume={6},
number ={2},
pages={314-332},
year={1988}
}


@INPROCEEDINGS{Bonastre2004,
author = {J. F. Bonastre and N. Scheffer and C. Fredouille and D. Matrouf},
title = {{N}IST04 speaker recognition evaluation campaign: new LIA speaker detection platform based on ALIZE toolkit},
booktitle={Proc. of NIST 2004 speaker recognition workshop},
year = {2004}
}

@INPROCEEDINGS{kenny2014,
author ={P. Kenny and T. Stafylakis and  P. Ouellet and   M. J. Alam and  P. Dumouche},
title = {{S}upervised/Unsupervised Voice Activity Detectors for Text-dependent Speaker Recognition on the RSR2015 Corpus},
booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
year = {2014}
}

@Article{Gerkmann2012,
author ={T. Gerkmann and R.C. Hendriks},
title ={{U}nbiased  MMSE-based noise power estimation with low complexity and low tracking delay},
journal={IEEE Trans. on Audio, Speech and Language Processing},
pages={1383-1393},
volume = {20},
year ={2012}
}

@Article{Hu2012b,
author ={D. L. Hu and others},
title = {{V}oice Activity Detection with Decision Trees in Noisy Environments},
journal ={Applied Mechanics and Materials},
volume ={128-129},
pages = {749-752},
year = {2012}
}


@inproceedings{Khoury+2016,
author={E. Khoury and M. Garland},
title={I-Vectors for speech activity detection},
year={2016},
booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
pages={334-339}
}

@inproceedings{Kinnunen+2016,
author={T. Kinnunen and A. Sholokhov and E. Khoury and D. A. Lehmann Thomsen and M. Sahidullah and Z.-H Tan},
title={HAPPY Team Entry to NIST OpenSAD Challenge: A Fusion of Short-Term Unsupervised and Segment i-Vector Based Speech Activity Detectors},
year={2016},
booktitle={Proc. of Interspeech},
pages={2992-2996}
}

@Article{Deka_ieee2011,
       author= {N. Dehak and P. Kenny and R. Dehak and  P. Dumouchel and
               P. Ouellet},
       title= {{F}ront-End Factor Analysis for Speaker Verification},
       journal={IEEE Trans. on Audio, Speech and Language Processing},
       volume={19},
       pages={788-798},
       year = {2011}
}

@Article{reynold95,
  author="D. A. Reynolds",
  title="{S}peaker Identification and Verification using Gaussian Mixture Speaker Models",
  journal="Speech Communication",
  volume="17",
  pages="91-108",
  year="1995"
}

@inproceedings{Hirsch2000,
author ={ H.-G. Hirsch and D. Pearce},
title = {{T}HE AURORA EXPERIMENTAL FRAMEWORK FOR THE PERFORMANCE EVALUATION OF SPEECH RECOGNITION SYSTEMS UNDER NOISY CONDITIONS},
booktitle ={Automatic Speech Recognition: Challenges for the Next Millennium, ISCA ITRW ASR2000},
year= {2000}
}

@INPROCEEDINGS{Pelecanos01,
       author={J. Pelecanos and S. Sridharan},
       title={{F}eature {W}arping for {R}obust {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={213-218},
       year= {2001}
}

@inproceedings{PlchotMMDMCGHMMSSTTZZ13,
  author    = {Oldrich Plchot and
               Spyros Matsoukas and
               Pavel Matejka and
               Najim Dehak and
               Jeff Z. Ma and
               Sandro Cumani and
               Ondrej Glembek and
               Hynek Hermansky and
               Sri Harish Reddy Mallidi and
               Nima Mesgarani and
               Richard M. Schwartz and
               Mehdi Soufifar and
               Zheng{-}Hua Tan and
               Samuel Thomas and
               Bing Zhang and
               Xinhui Zhou},
  title     = {{D}eveloping a speaker identification system for the {DARPA} {RATS}
               project},
  booktitle = {Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages     = {6768-6772},
  year      = {2013}
  }
  
 @misc{RATS, 
  title ="https://www.darpa.mil/program/robust-automatic-transcription-of-speech"
  }
  
  @inproceedings{LDC_rats,
  author={K. Walker and X. Ma and D. Graff and S. Strassel and S. Sessa and K. Jones},
  title={{R}ATS Speech Activity Detection},
  booktitle={ LDC2015S02. Hard Drive. Philadelphia: Linguistic Data Consortium},
  year={2015},
  url="https://catalog.ldc.upenn.edu/ldc2015s02"
  }
  
 @inproceedings{Gonzalez2011, 
   author = {S. Gonzalez and M. Brookes},
   title = {{A} pitch estimation filter robust to high levels of noise (PEFAC)},
   booktitle= {Proc. of {EUSIPCO}},
   pages={451-455},
   year = {2011}
   }
   
@Article{RSR2015,
author={A. Larcher and  K. A. Lee and  B. Ma and H. Li},
title= {{T}ext-dependent {S}peaker {V}erification: {C}lassifiers, {D}atabases and {RSR2015}},
journal={Speech Communication},
volume={60},
pages={56-77},
year={2014}
}
  
@Article{Sadjadi2013,  
  author={S. Sadjadi and J. H. L. Hansen},
  title={{U}nsupervised speech activity detection using voicing measures and perceptual spectral flux},
  journal={IEEE Signal Processing Letters},
  volume={20},
  number={3},
  pages={197-200},
  year={2013}
  }
  
  @article{petsatodis2011convex,
  title={Convex combination of multiple statistical models with application to VAD},
  author={Petsatodis, Theodoros and Boukis, Christos and Talantzis, Fotios and Tan, Zheng-Hua and Prasad, Ramjee},
  journal={IEEE Transactions on Audio, Speech, and Language Processing},
  volume={19},
  number={8},
  pages={2314--2327},
  year={2011},
  publisher={IEEE}
}
  @article{zhang2013deep,
  title={Deep belief networks based voice activity detection},
  author={Zhang, Xiao-Lei and Wu, Ji},
  journal={IEEE Transactions on Audio, Speech, and Language Processing},
  volume={21},
  number={4},
  pages={697--710},
  year={2013},
  publisher={IEEE}
}
  
  
  @misc{RedDots,
title= {The RedDots Challenge: Towards Characterizing Speakers from Short Utterances},
howpublished ={https://sites.google.com/site/thereddotsproject/reddots-challenge}
}

@inproceedings{wu2015,
author={Z. Wu and T. Kinnunen and N. Evans and J. Yamagishi and C. Hanilci and
M. Sahidullah and A. Sizov},
title={{ASV}spoof 2015: the {F}irst {A}utomatic {S}peaker {V}erification {S}poofing and {C}ountermeasures challenge},
booktitle={Proc. of Interspeech},
pages={2037-2041},
year ={2015}
}
 
 @INPROCEEDINGS{Timit,
author = {J. S. Garofolo and L. F. Lamel and W. M. Fisher and J. G. Fiscus and  D. S. Pallett and N. L. Dahlgren and V. Zue},
title = {{TIMIT} {A}coustic-{P}honetic {C}ontinuous {S}peech {C}orpus {LDC}93{S}1},
publisher = {Web Download. Philadelphia: Linguistic Data Consortium},
year={1993}
}


@Article{htkbook,
  author="S. Young and D. Kershaw and J. Odell and V. Valtchev and P. Woodland and et al.",
  title="{HTK} {B}ook",
  journal="Copyright 2001-2006 CUED"
   }


@Article{zt2017_isorobot,
author ={Z.-H. Tan and N. B. Thomsen and  X. Duan and  E. Vlachos and S. E. Shepstone and M. Højfeldt Rasmussen and  J. L. Højvang},
title ={{i}SocioBot: A Multimodal Interactive Social Robot},
journal ={International Journal of Social Robotics},
pages ={1-15},
year ={2017}
}

@INPROCEEDINGS{DBLP:journals/corr/DubeyMM16,
  author    = {Harishchandra Dubey and   Matthias R. Mehl and
               Kunal Mankodiya},
  title     = {BigEAR: Inferring the Ambient and Emotional Correlates from Smartphone-based Acoustic Big Data},
  booktitle   = {International Workshop on Big Data Analytics for Smart and Connected},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.03636}
  }
 
@INPROCEEDINGS{Semwal2017,
  	author={N. Semwal and A. Kumar and S. Narayanan},
    title={{A}utomatic speech emotion detection system using multi-domain acoustic feature selection and classification models},
    booktitle= {Identity, Security and Behavior Analysis (ISBA)},
    year={2017}
    }
    
@INPROCEEDINGS{Chorianopoulou2016,
author ={ A. Chorianopoulou and P. Koutsakis and A. Potamianos},
title = {{S}peech Emotion Recognition Using Affective Saliency},
booktitle={Proc. of Interspeech},
pages={500-504},
year ={2016}
}

@INPROCEEDINGS{Stefanus2017,
author = {I. Stefanus and R. S. J. Sarwono and M. I. Mandasari},
title = {{G}MM based automatic speaker verification system development for forensics in Bahasa Indonesia},
booktitle ={Proc. of Instrumentation, Control, and Automation (ICA)},
year={2017}
}

@INPROCEEDINGS{Nautsch2016,
author ={A. Nautsch and R. Bamberger and C. Busch},
title={{D}ecision Robustness of Voice Activity Segmentation in Unconstrained Mobile Speaker Recognition Environments},
booktitle ={Proc. of Biometrics Special Interest Group (BIOSIG)},
year={2016}
}

@INPROCEEDINGS{Dhanush2017,
author ={B. K. Dhanush and others},
title ={{F}actor analysis methods for joint speaker verification and spoof detection},
booktitle ={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2017}
}


@inproceedings{Tao2017,
  author={Fei Tao and Carlos Busso},
  title={Bimodal Recurrent Neural Network for Audiovisual Voice Activity Detection},
  year=2017,
  booktitle={Proc. of Interspeech},
  pages={1938-1942}
 }

@inproceedings{Ferrer2016,
author={L. Ferrer and M. Graciarena and V. Mitra},
title={{A} phonetically aware system for speech activity detection},
booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages={5710-5714},
year ={2016}
}



@inproceedings{Zazo+2016,
author={Ruben Zazo and Tara N. Sainath and Gabor Simko and Carolina Parada},
title={Feature Learning with Raw-Waveform CLDNNs for Voice Activity Detection},
year=2016,
booktitle={Proc. of Interspeech},
pages={3668--3672}
}


@Article{Gerkmann2013,
author={T. Gerkman and R. C. Hendriks},
title = {{U}nbiased MMSE-Based Noise Power Estimation With Low Complexity and Low Tracking Delay},
journal ={IEEE Trans Audio, Speech, Language Processing},
volume={20},
pages={1383-1393},
year={2012}
}

@Article{Ephraim1984,
author = {Y. Ephraim and D. Malah},
title={{S}peech enhancement using a minimum mean-square error short-time spectral amplitude estimator},
journal ={ IEEE Trans. on Acoust., Speech, Signal Processing},
volume ={32},
pages={1109-1121},
year={1984}
}

@Article{Kolbk2017a,
author = {M. Kolb$\ae$k and Z.-H. Tan and J. Jensen},
title = {{S}peech Intelligibility Potential of General and Specialized Deep Neural Network based Speech Enhancement Systems},
journal = {IEEE/ACM Trans.  on Audio, Speech and Language Processing},
volume={25},
number={1},
pages={153-167},
year={2017}
}

@inproceedings{Michelsanti2017,
  author={D. Michelsanti and Z.-H. Tan},
  title={{C}onditional Generative Adversarial Networks for Speech Enhancement and Noise-Robust Speaker Verification},
  year=2017,
  booktitle={Proc. of Interspeech},
  pages={2008-2012}
  }

@inproceedings{Wang2017a,
author = {X. Zhang and Z.-Q. Wang and D.L. Wang},
title = {{A} speech enhancement algorithm by iterating single- and multi-microphone processing and its application to robust ASR},
booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages = {276-280},
year={2017}
}

@inproceedings{Kolbk2016a,
author = {M. Kolb$\ae$k and Z.-H. Tan and J. Jensen},
title = {{S}peech enhancement using long short-term memory based recurrent neural networks for noise robust speaker verification},
booktitle ={Proc. of Spoken Language Technology Workshop (SLT)},
year={2016},
pages={305-311},
}
@Article{Jensen2015a,
author = {J. Jensen and Z.-H. Tan},
title={{M}inimum Mean-Square Error Estimation of Mel-Frequency Cepstral Features},
journal={IEEE/ACM Trans.  Audio, Speech and Language Processing},
volume={23},
number={1},
pages={186-197},
year={2015}
}


@Article{Hermanksy94,
       author = {H. Hermanksy and N. Morgan},
       title = {{R}ASTA Processing of Speech},
       journal={IEEE Trans. on Speech and Audio Processing},
       volume={2},
       pages={578-589},
       year={1994}
}

@techreport{G191,
author ={G. 191},
title = {{S}oftware tools for speech and audio coding standardization},
institution ={International Telecommunication Union},
year = {2005}
}

@inproceedings{kinnunen2013practical,
  title={{A} practical, self-adaptive voice activity detector for speaker verification with noisy telephone and microphone data.},
  author={Kinnunen, Tomi and Rajan, Padmanabhan},
  booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages={7229--7233},
  year={2013}
}

@inproceedings{tan2008posteriori,
  title={{A} posteriori SNR weighted energy based variable frame rate analysis for speech recognition},
  author={Tan, Zheng-Hua and Lindberg, B{\o}rge},
  booktitle={Proc. of Interspeech},
  pages={1024-1027},
  year={2008}
}

@inproceedings{petsatodis2011multi,
  title={{M}ulti-sensor voice activity detection based on multiple observation hypothesis testing},
  author={Petsatodis, Theodoros and Talantzis, Fotios and Boukis, Christos and Tan, Zheng-Hua and Prasad, Ramjee},
  booktitle={Proc. of Interspeech},
  pages={2633-2636},
  year={2011}
}

@inproceedings{ferrernoise2013,
  title={{A} Noise-Robust System for NIST 2012 Speaker Recognition Evaluation},
  author={Ferrer, L. and McLaren, M. and Scheffer, N. and Lei, Y. and Graciarena, M. and Mitra, V.},
  booktitle={Proc. of Interspeech},
  year={2013},
  pages={1981-1985}
}

@inproceedings{chuangsuwanich2011robust,
  title={{R}obust voice activity detector for real world applications using harmonicity and modulation frequency},
  author={Chuangsuwanich, Ekapol and Glass, James},
  booktitle={Proc. of Interspeech},
  pages={2645-264},
  year={2011}
}

@article{price2018low,
  title={A Low-Power Speech Recognizer and Voice Activity Detector Using Deep Neural Networks},
  author={Price, Michael and Glass, James and Chandrakasan, Anantha P},
  journal={IEEE Journal of Solid-State Circuits},
  volume={51},
  number={1},
  pages={66-75},
  year={2018},
  publisher={IEEE}
}

@article{sholokhov2018semi,
  title={Semi-supervised speech activity detection with an application to automatic speaker verification},
  author={Sholokhov, Alexey and Sahidullah, Md and Kinnunen, Tomi},
  journal={Computer Speech \& Language},
  volume={47},
  pages={132--156},
  year={2018},
  publisher={Elsevier}
}

@article{shepstone2013audio,
  title={Audio-based age and gender identification to enhance the recommendation of TV content},
  author={Shepstone, Sven and Tan, Zheng-Hua and Jensen, Soren},
  journal={IEEE Transactions on Consumer Electronics},
  volume={59},
  number={3},
  pages={721--729},
  year={2013},
  publisher={IEEE}
}

@inproceedings{zhao2017two,
  title={A two-stage algorithm for noisy and reverberant speech enhancement},
  author={Zhao, Yan and Wang, Zhong-Qiu and Wang, DeLiang},
  booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages={5580--5584},
  year={2017},
  organization={IEEE}
}

@phdthesis{lee2014discovering,
  title={Discovering linguistic structures in speech: Models and applications},
  author={Lee, Chia-Ying},
  year={2014},
  school={Massachusetts Institute of Technology}
}

@misc{NIST2016SRE,
title= {Speaker Recognition Evaluation 2016},
howpublished ={https://www.nist.gov/itl/iad/mig/speaker-recognition-evaluation-2016}
}

@article{hermansky1994rasta,
  title={RASTA processing of speech},
  author={Hermansky, Hynek and Morgan, Nelson},
  journal={IEEE transactions on speech and audio processing},
  volume={2},
  number={4},
  pages={578--589},
  year={1994},
  publisher={IEEE}
}

@article{yang2016voice,
  title={Voice activity detection algorithm based on long-term pitch information},
  author={Yang, Xu-Kui and He, Liang and Qu, Dan and Zhang, Wei-Qiang},
  journal={EURASIP Journal on Audio, Speech, and Music Processing},
  volume={2016},
  number={1},
  pages={14},
  year={2016},
  publisher={Nature Publishing Group}
}

@inproceedings{shao2018use,
  title={Use of Pitch Continuity for Robust Speech Activity Detection},
  author={Shao, Yiwen and Lin, Qiguang},
  booktitle={2018 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={5534--5538},
  year={2018},
  organization={IEEE}
}

@book{loizou2013speech,
  title={Speech enhancement: theory and practice},
  author={Loizou, Philipos C},
  year={2007},
  publisher={CRC press}
}

@article{ssgmm-sad-2017,
title = "Semi-supervised speech activity detection with an application to automatic speaker verification",
author = "Alexey Sholokhov and Md Sahidullah and Tomi Kinnunen",
journal = "Computer Speech \& Language",
volume = "47",
number = "",
pages = "132 - 156",
year = "2018",
}

@inproceedings{VQVAD,
author={T. Kinnunen and P. Rajan},
title={{A} practical, self-adaptive voice activity detector for speaker verification with noisy telephone and microphone
data},
booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2013}
}

@inproceedings{SF_vad2019,
author={M. Moattar and M. M. Homayounpour},
title={{A} Simple But Efficient Real-Time Voice Activity Detection Algorithm},
booktitle={Proc. of  EUSIPCO},
year={2009},
pages={2549-2553}
}

@inproceedings{PNCC2012,
author={C. Kim and R. Stern},
title={{P}ower-normalized cepstral coefficients (PNCC) for robust speech recognition},
booktitle={Proc. of  IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2012},
pages={4101-4104}
}

@misc{Ellis05-rastamat,
      Author = {D. P. W. Ellis},
      Year = {2005},
      Title = {{PLP} and {RASTA} (and {MFCC}, and inversion) in {M}atlab},
      Url = {http://www.ee.columbia.edu/~dpwe/resources/matlab/rastamat/},
      Note = {online web resource}}
}

@inproceedings{Yaafe,
author={B.Mathieu and S.Essid and T.Fillon and J.Prado and G.Richard}, 
booktitle={{Y}AAFE, an Easy to Use and Efficient Audio Feature Extraction Software},
booktitle={Proc. of the ISMIR conference},
year = {2010}
}


